Analysis note: measurement of energy-energy correlator in $e^{+}e^{-}$ collisions at $91$ GeV with archived ALEPH data

Electron-positron ($e^+e^-$) collisions provide a clean environment for precision tests of Quantum Chromodynamics (QCD) due to the absence of hadronic initial-state effects. We present a novel analysis of archived ALEPH data from the Large Electron-Positron Collider at the $Z$ pole, leveraging energy-energy correlators (EECs) to study hadronic energy flow with unprecedented precision. The two-point EEC is measured as a function of the angular separation between particles spanning from the collinear to the back-to-back limits in a remarkably differential test of perturbative and non-perturbative QCD. The results are consistent with previous LEP measurements and provide significantly improved precision and finer angular binning resolution, especially at small angles and in the back-to-back limit. Comparisons with \textsc{pythia} 6 simulations show overall agreement, with deviations in key kinematic regions offering insights into hadronization. The measurement performed here connects to new opportunities for precision QCD studies in archived and future collider data.

==> SomeStuffsFrom2PCLEP2Analysis/lep2evtsel.tex <==
% \section{Event Selection}
% \label{sec:EvtSelection}
%%%%% data subset (1. Z-resonance, 2. high-energy)
The analysis is performed using the data sample taken by the ALEPH detector from 1992 to 2000, corresponding to collision energies of $\sqrt{s} = 91$--209~GeV and a total integrated luminosity of 745~pb$^{-1}$ of data. 
We have divide the data into two datasets according to their center-of-mass energies. One is the {\it $Z$-resonance dataset}, which provides results extending the previous measurement with only LEP-I data~\cite{Badea:2019vey}. The other one focuses exclusively on {\it high-energy events} at LEP-II, with collision energies greater than those of the $Z$-boson mass.

%%%%% - data subset (2.1 qq-like, 2.2 WW-like)
%%%%% -  Event selections:
%%%%% https://github.com/yenjie/StudyMult/blob/master/DataProcessing/include/eventSelection.h#L160
Unlike the sample taken at the 91.2 GeV, where $Z$-decays dominate over other processes, a wide variety of processes beyond the $e^+e^- \to q\bar{q}$ fragmentation also make non-negligible contributions to the high-energy sample. The initial-state QED radiation is significant in high-energy events, an effect called ``radiative-return-to-$Z$.'' We follow the selection criteria studied by the ALEPH collaboration~\cite{ALEPH:2003obs}. To ensure that the analyzed events are produced from high center-of-mass energy collisions, we calculate the effective center-of-mass energy ($\sqrt{s'}$) by clustering the event into two jets, and obtain
\begin{equation}
s' = \frac{\sin \theta_1 + \sin \theta_2 - | \sin(\theta_1 + \theta_2) |}{ \sin \theta_1 + \sin \theta_2 + | \sin(\theta_1 + \theta_2) | } \times s,
\end{equation}
where $\theta_{1,2}$ are the angles of the two jets with respect to the beam (or the $z$) direction.
With the clustered two jets, the visible two-jet invariant-mass ($M_{\rm vis}$) can be calculated and also be used as a useful variable to suppress the QED radiation background.
In the analysis, the $\sqrt{s'}$ is required to be greater than $0.9 \sqrt{s}$, and $M_{\rm vis}$ should be larger than $0.7 \sqrt{s}$.

==> SomeStuffsFrom2PCLEP2Analysis/lep2mc.tex <==

Different MC processes are weighted according to the cross-sections calculated by event generators. In Table~\ref{tab:physics_processes}, we show the number of simulated events and the corss-sections associated to different MC processes in the collision energy $\sqrt{s}=207$~GeV. Different collision-energy benchmarks: $\sqrt{s}=183,187,192,196,200,202,205,207$~GeV are used for the full LEP-II analysis.
%\txcb{Talk about more details?}\txcb{YJ: probably include the physics processes that we studied with MC in a table?}

\begin{table}[h]
\centering
\caption{List of physics processes with Monte Carlo event counts and cross-sections for LEP-II analysis. Shown in the table is the simulation with a collision energy $\sqrt{s}=207$~GeV. }
\begin{tabular}{|c|l|r|r|}
\hline
TAG & Process & \# Events & Cross-Section (picobarns) \\
\hline
\multicolumn{4}{|c|}{\(\gamma\gamma \rightarrow \text{hadrons}\)} \\
\hline
GGUD & \( \gamma\gamma  \rightarrow uu/dd \) & 2,000,000 & \( 1795.310 \pm 1.847 \) \\
GGSS & \( \gamma\gamma  \rightarrow ss \) & 200,000 & \( 88.486 \pm 0.287 \) \\
GGCC & \( \gamma\gamma  \rightarrow cc \) & 700,000 & \( 271.910 \pm 0.457 \) \\
GGBB & \( \gamma\gamma  \rightarrow bb \) & 25,000 & \( 1.410 \pm 0.012 \) \\
\hline
\multicolumn{4}{|c|}{\( e^+e^- \rightarrow \text{hadrons} \)} \\
\hline
KQQ  & \( e^+e^- \rightarrow qq \) & 2,000,000 & \( 81.007 \pm 0.022 \) \\
TT   & \( e^+e^- \rightarrow \tau^+\tau^- \) & 100,000 & \( 6.742 \pm 0.007 \) \\
\hline
\multicolumn{4}{|c|}{\( e^+e^- \rightarrow 4f \)} \\
\hline
KWW4F & \( W^+W^- \) & 2,350,000 & \( 18.958 \pm 0.005 \) \\
KWENU & \( W e \nu \) & 100,000 & \( 0.774 \pm 0.001 \) \\
PZEE  & \( Z e e \) & 200,000 & \( 8.470 \pm 0.019 \) \\
PZZ   & \( ZZ \) & 200,000 & \( 2.340 \pm 0.005 \) \\
ZNN   & \( Z \nu\nu \) & 50,000 & \( 0.017 \pm 0.000 \) \\
\hline
\end{tabular}
\label{tab:physics_processes}
\end{table}

==> SomeStuffsFrom2PCLEP2Analysis/lep2mult_thrust.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% multiplicity %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Event multiplicity distribution}

After applying all the selection criteria, the subsequent offline multiplicity, denoted as \({\rm N}_{\rm Trk}^{\rm Offline}\), is used for studying the correlation function's multiplicity dependence. It is important to note that \({\rm N}_{\rm Trk}^{\rm Offline}\) represents the count of charged particles that have passed the selection criteria outlined in the ``Charged particle selection'' subsection~\ref{sec:chgdSel}, without any additional efficiency corrections.

Figure~\ref{fig:NtrkOffline} displays the offline multiplicity distributions in data collected at various collision energies. In the low-multiplicity region, there is a residual contribution from QED ($e^+e^- \to \tau^+\tau^-$) and two-photon events. However, these are significantly suppressed due to the hadronic event selection. Above the $W^{+}W^{-}$ production threshold ($\sqrt{s} > 160$~GeV), four-fermion processes mediated by either single or double $W$ or $Z$ bosons serve as sub-dominant channels in hadronic decays. At the highest multiplicity, four-fermion processes, especially $W^{+}W^{-}$ production, emerge as the dominant channels.

The multiplicity classes used in this study, along with their corresponding fraction of data, and the mapping of average offline multiplicities $\langle {\rm N}_{\rm Trk}^{\rm Offline}\rangle$ to average multiplicities after efficiency correction $\langle {\rm N}_{\rm trk}^{\rm corr}\rangle$ are listed in Table~\ref{tab:NtrkCorr}. 



\begin{figure}[ht]
\centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/183_nTrkOffline.pdf}
        \caption{$\sqrt{s}=183$~GeV (Year 1997)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/189_nTrkOffline.pdf}
        \caption{$\sqrt{s}=189$~GeV (Year 1998)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/192_nTrkOffline.pdf}
        \caption{$\sqrt{s}=192$~GeV (Year 1999)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/196_nTrkOffline.pdf}
        \caption{$\sqrt{s}=196$~GeV (Year 1999)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/200_nTrkOffline.pdf}
        \caption{$\sqrt{s}=200$~GeV (Year 1999)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/202_nTrkOffline.pdf}
        \caption{$\sqrt{s}=202$~GeV (Year 1999)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/205_nTrkOffline.pdf}
        \caption{$\sqrt{s}=205$~GeV (Year 2000)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/207_nTrkOffline.pdf}
        \caption{$\sqrt{s}=207$~GeV (Year 2000)}
        %\label{fig:}
    \end{subfigure}
\caption{The offline multiplicity (\ntrkoff) distributions for high-energy events from different years. 
Data are presented as black error bars; stacked histograms show the decomposition of different simulated processes scaled according to the calculated cross-sections.
}
\label{fig:NtrkOffline}
\end{figure}

\begin{figure}[ht]
\centering
     \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/183_thrust.pdf}
        \caption{$\sqrt{s}=183$~GeV (Year 1997)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/189_thrust.pdf}
        \caption{$\sqrt{s}=189$~GeV (Year 1998)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/192_thrust.pdf}
        \caption{$\sqrt{s}=192$~GeV (Year 1999)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/196_thrust.pdf}
        \caption{$\sqrt{s}=196$~GeV (Year 1999)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/200_thrust.pdf}
        \caption{$\sqrt{s}=200$~GeV (Year 1999)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/202_thrust.pdf}
        \caption{$\sqrt{s}=202$~GeV (Year 1999)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/205_thrust.pdf}
        \caption{$\sqrt{s}=205$~GeV (Year 2000)}
        %\label{fig:}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,angle=0]{figures/nTrkOfflineContributions/207_thrust.pdf}
        \caption{$\sqrt{s}=207$~GeV (Year 2000)}
        %\label{fig:}
    \end{subfigure}
\caption{The thrust distributions for high-energy events from different years. 
Data are presented as black error bars; stacked histograms show the decomposition of different simulated processes scaled according to the calculated cross-sections.
}
\label{fig:Thrust}
\end{figure}
\begin{figure}[ht]
\centering
     \begin{subfigure}[b]{\textwidth}
     \centering
        \includegraphics[width=0.40\textwidth]{figures/nTrkOfflineLEP2ContributionsBySources/nTrkOffline_logy_total.pdf}
        \includegraphics[width=0.40\textwidth]{figures/nTrkOfflineLEP2ContributionsBySources/thrust_logy_total.pdf}
        \caption{Merged LEP-II sample}
        %\label{fig:}
    \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%     \centering
%        \includegraphics[width=0.40\textwidth]{figures/nTrkOfflineLEP2ContributionsBySources/nTrkOffline_logy_qqLike.pdf}
%        \includegraphics[width=0.40\textwidth]{figures/nTrkOfflineLEP2ContributionsBySources/thrust_logy_qqLike.pdf}
%        \caption{$q\bar{q}$-like}
        %\label{fig:}
%    \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%     \centering
%        \includegraphics[width=0.40\textwidth]{figures/nTrkOfflineLEP2ContributionsBySources/nTrkOffline_logy_WWLike.pdf}
%        \includegraphics[width=0.40\textwidth]{figures/nTrkOfflineLEP2ContributionsBySources/thrust_logy_WWLike.pdf}
%        \caption{$WW$-like}
        %\label{fig:}
%    \end{subfigure}
\caption{The multiplicity and thrust distributions of high-energy events of years 1997-2000. 
%%%%%% E130-E209_Y1995-Y2000: full LEP2 results, but we don't have simulation in √s=130 GeV, so that the data-MC agreement is not that good
%%%%%% E183-E209_Y1997-Y2000: better data-MC agreement
Data are presented as black error bars; stacked histograms show the decomposition of different simulated processes scaled according to the calculated cross-sections.
}
\label{fig:HighEnergySampleBySources}
\end{figure}

\begin{figure}[ht]
\centering
     \centering
        \includegraphics[width=0.40\textwidth]{figures/LEP1cfLEP2/nTrkOffline_logyLEP1nLEP2.pdf}
        \includegraphics[width=0.40\textwidth]{figures/LEP1cfLEP2/thrust_logyLEP1nLEP2.pdf}
        %\label{fig:}
\caption{The comparison of $Z$-resonance's and high-energy's multiplicity and thrust distributions. 
}
\label{fig:LEP1cfLEP2}
\end{figure}

\begin{table}[ht]
\caption{Average multiplicities and corrected multiplicities of different \ntrkoff intervals for the LEP-I and LEP-II datasets.}
\begin{center}
\footnotesize
\begin{tabularx}{\textwidth}{
    >{\centering}p{0.08\textwidth} | 
    >{\centering}p{0.12\textwidth}
    >{\centering}p{0.09\textwidth}
    >{\centering}p{0.09\textwidth} |
    >{\centering}p{0.08\textwidth} | 
    >{\centering}p{0.12\textwidth}
    >{\centering}p{0.09\textwidth}
    X
}
\hline\hline
\multirow{2}{*}{\parbox{0.09\textwidth}{\ntrkoff interval}} &
\multicolumn{3}{c|}{LEP-I} & 
\multicolumn{1}{c|}{\multirow{2}{*}{\parbox{0.09\textwidth}{\ntrkoff interval}}} &
\multicolumn{3}{c}{LEP-II} \\
\cline{2-4} \cline{6-8}
&  Fraction (\%) & $\left<{\rm N}_{\rm Trk}^{\rm Offline}\right>$ & $\left<{\rm N}_{\rm trk}^{\rm corr}\right>$ &
&   Fraction (\%) & $\left<{\rm N}_{\rm Trk}^{\rm Offline}\right>$ & $\left<{\rm N}_{\rm trk}^{\rm corr}\right>$ \\
\hline 
$[5,10)$        & 3.1 & 8.2 & 8.9 & $[10,20)$       & 58.6 & 15.2 & 17.3\\
$[10,20)$       & 59.2 & 15.2 & 15.8 & $[20,30)$       & 33.1 & 23.1 & 25.7 \\
$[20,30)$       & 34.6 & 23.1 & 23.4 & $[30,40)$       & 3.7 & 32.6 & 35.9 \\
$[30,\infty)$   & 3.1 & 32.4 & 32.6 & $[40,50)$       & 0.4 & 42.8 & 47.1 \\
$[35,\infty)$   & 0.5 & 36.9 & 37.2 & $[50,\infty)$   & $<$0.1 & 53.0 & 58.4\\
\hline\hline
\end{tabularx}
\label{tab:NtrkCorr}
\end{center}
\end{table} 

\subsection{Event thrust}
\label{sec:Thrust}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% thrust %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The event thrust axis~\cite{PhysRevLett.39.1587} is obtained through maximizing the sum of the projected particle momenta on itself in the center-of-mass frame, formulating as
\begin{equation}
\hat{n} \equiv max_{\hat{n}} \frac{\sum\nolimits_{i} \left| \Vec{p_i} \cdot \hat{n} \right|}{\sum\nolimits_{i} \left| \Vec{p_i} \right|},
\label{eqn:Thrust}
\end{equation}
where $\hat{n}$ is the resulting event thrust axis and $\Vec{p_i}$ is the momentum of the $i$-th particle, extending over charged, neutral particles and the missing transverse momentum. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% neutrals %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Neutral particles are energy flow candidates from the ECAL and HCAL. Requirements on the detector acceptance of $|\cos\theta| < 0.98$ and a cluster energy greater than 0.4~GeV are applied.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% MET %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The invisible objects, such as neutrinos, and non-reconstructed particles at the reconstruction level, are taken into accounts as the missing momentum in the calculation of the event thrust, given by
\begin{equation}
\Vec{p}_{\rm MET} = -\sum\nolimits_{\rm neu, chg} \Vec{p}.
\label{eqn:MissP}
\end{equation}


In Figure~\ref{fig:HighEnergySampleBySources} we compare the offline multiplicity distributions and the thrust distributions for the merged LEP-II sample. 

%and for events with the \qq-like and \WW-like topology selections. 
The MC simulation provides an excellent description of the data. While the $q\bar{q}$ final states dominant the lower multiplicity range, $W^{+}W^{-}$ contribution increases with \ntrkoff and becomes the most significant contribution at high multiplicity.

Figure~\ref{fig:LEP1cfLEP2} shows the offline multiplicity and the thrust distributions in data collected at different collision energies. The high-energy sample provides a significantly higher multiplicity reach compared to the $Z$-resonance sample. The thrust distribution of the high-energy sample is also comparably more spherical as opposed to the $Z$-resonance sample due to the larger contribution of multi-jets in the final state in LEP-II than LEP-I.

==> SomeStuffsFrom2PCLEP2Analysis/syst2pc.tex <==
We consider the systematic uncertainties due to the event and track selections, the $B(0,0)$ normalization factor, and the residual MC correction operations on the long-range associated yield $Y_l(\Delta \phi)$.
% We utilized the systematics assessment established in the two-particle correlation analysis work with ALEPH LEP-I archived data~\cite{Badea:2019vey}. We also summarize both the old (LEP-I) values and the new LEP-II results for a comprehensive view in this analysis note.

We consider variations on the ISR and the hadronic event selection criteria for the event selections. 
We vary the ISR selections by relaxing the requirement on the visible two-jet invariant mass $M_{\rm vis}$ from the nominal cut point $0.7\sqrt{s}$ to $0.65\sqrt{s}$, and relaxing the effective center-of-mass energy $\sqrt{s'}$ from $0.9\sqrt{s}$ to $0.87\sqrt{s}$. Two variations give consistent results. The larger uncertainties among the two are quoted as the final uncertainty values.
For the hadronic event selections, the same treatment as the LEP-I work is adopted. We examine their systematic effect by varying the requirements on the number of particles and the reconstructed charged-particle energy. The selection criteria are changed from a $13$ minimal number of particles to $10$ for an event and from $15$~GeV minimal reconstructed charged-particle energy to $10$~GeV. Overall, the hadronic event selections and ISR selections are correlated. The difference from the variation of ISR selections is significantly more prominent. Hence, it is reported as the final event selection uncertainty.
For the track selection, we changed the number of track hits in the time projection chamber from 4 hits to 7 hits.
The inclusion of the $B(0,0)$ factor as the normalization choice (in eq.~\ref{eqn:2PC}) also introduces a systematic uncertainty. We evaluate its impact based on the statistical uncertainty of the $B(0,0)$ normalization factor.
The above systematic uncertainties, in general, impact uniformly across \dphi bins.

The residual MC correction factor (in Section~\ref{sec:residMCCorr}) can lead to an uncorrelated uncertainty across \dphi bins. This systematic uncertainty is estimated by attempting different fits on the residual MC correction factor. Three different functional forms are considered, with half of the maximum deviation between fits considered as the uncertainty from the residual MC correction.

In Table~\ref{tab:Systematics_beam} and~\ref{tab:Systematics_thrust}, the systematic uncertainties due to the aforementioned systematic sources as a function of \ntrk are shown for the beam-axis and thrust-axis analyses, respectively. All numbers are given as percentages. For the systematic evaluation of the Bayesian analysis, we vary the number of toy samples in a pseudo-dataset from 50k to 100k, and vary the granularity of a 1000-step parameter scanning from a 10-sigma interval $[x-10\sigma_x, x+10\sigma_x]$ to a 5-sigma interval $[x-5\sigma_x, x+5\sigma_x]$.

\begin{table}[ht] % systematic table beam
\footnotesize
\caption{Beam axis analysis systematic uncertainties for the LEP-I and LEP-II data as a function of the offline multiplicity \ntrkoff. All values are reported as percentages of the long-range differential associated yield. The systematic uncertainties for LEP-I measurement are from the published two-particle correlation analysis with ALEPH archived data~\cite{Badea:2019vey}. Note that in the residual MC correction column, we report the maximum deviation value between fits. The final considered systematic uncertainty is a half of the maximum deviation.}
\begin{center}
\begin{tabularx}{\textwidth}{C|CCCC}
\hline\hline
\hspace{0.2cm}\ntrkoff \hspace{0.2cm} & TPC hits  & Event energy and track cuts     & $B(0,0)$  & Residual MC correction \\
\hline
\multicolumn{5}{c}{LEP-I}\\
\hline 
$[ 5,10)$ & 0.7 & 0.6 & 0.11 & 10.3 \\
\hline
$[10,20)$ & 0.7 & 0.0 & 0.015 & 2.3 \\
\hline
$[20,30)$ & 0.7 & 0.0 & 0.013 & 0.2 \\
\hline
$[30,\infty)$ & 0.7 & 0.0 & 0.027 & 1.2 \\
\hline
$[35,\infty)$ & 0.7 & 0.0 & 0.057 & 4.4 \\
\hline
\multicolumn{5}{c}{LEP-II}\\
\hline 
$[10,20)$ & 0.28 & 6.84 & 0.10 & 1.52 \\
\hline
$[20,30)$ & 1.99 & 2.97 & 0.06 & 0.61 \\
\hline
$[30,40)$ & 1.13 & 0.64 & 0.06 & 1.10 \\
\hline
$[40,50)$ & 0.45 & 0.10 & 0.09 & 1.50 \\
\hline
$[50,\infty)$ & 2.52 & 0.21 & 0.17 & 1.74 \\
\hline
\hline
\end{tabularx} 
\label{tab:Systematics_beam}
\end{center}
\end{table}

\begin{table}[ht] % systematic table thrust
\footnotesize
\caption{Thrust axis analysis systematic uncertainties for the LEP-I and LEP-II data as a function of the offline multiplicity \ntrkoff. All values are reported as percentages of the long-range differential associated yield. The systematic uncertainties for LEP-I measurement are from the published two-particle correlation analysis with ALEPH archived data~\cite{Badea:2019vey}. Note that in the residual MC correction column, we report the maximum deviation value between fits. The final considered systematic uncertainty is a half of the maximum deviation.}
\begin{center}
\begin{tabularx}{\textwidth}{C|CCCC}
\hline\hline
\hspace{0.2cm}\ntrkoff \hspace{0.2cm} & TPC hits  & Event energy and track cuts     & $B(0,0)$  & Residual MC correction \\
\hline
\multicolumn{5}{c}{LEP-I}\\
\hline 
$[ 5,10)$ & 0.3 & 3.4 & 0.88 & 0.50 \\
\hline
$[10,20)$ & 0.3 & 0.0 & 0.09 & 0.21 \\
\hline
$[20,30)$ & 0.3 & 0.0 & 0.05 & 0.06 \\
\hline
$[30,\infty)$ & 0.3 & 0.0 & 0.06 & 0.21 \\
\hline
$[35,\infty)$ & 0.3 & 0.0 & 0.13 & 0.21 \\
\hline
\multicolumn{5}{c}{LEP-II}\\
\hline 
$[10,20)$ & 1.09 & 0.39 & 0.44 & 1.17 \\
\hline
$[20,30)$ & 0.68 & 0.44 & 0.21 & 0.11 \\
\hline
$[30,40)$ & 0.65 & 0.05 & 0.12 & 0.10 \\
\hline
$[40,50)$ & 0.73 & 0.04 & 0.16 & 0.13 \\
\hline
$[50,\infty)$ & 1.60 & 0.50 & 0.27 & 0.02 \\
\hline
\hline
\end{tabularx} 
\label{tab:Systematics_thrust}
\end{center}
\end{table}

==> belle2sym.tex <==
%%%%%   Standard symbols for use in Belle II notes and papers. 
%%%%%
%%%%%	C. Hearty	21-Oct-2014		Based on babarsym.tex; authored by D. Hitlin, D. MacFarlane, P. Dauncey, and R. Waldi
%%%%%


\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% THE NAME OF THE COLLABORATION %%%%
\def\belletwo {Belle~II}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second 
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}





